Transport Properties of Anisotropic Polar Fluids: 1. Quadrupolar Interaction

Equilibrium molecular dynamics simulation and the Green-Kubo formalism were used to calculate self-diffusion coefficient, shear viscosity,and thermal conductivity for 30 different quadrupolar two-center Lennard-Jones fluids along the bubble line and in the homogeneous liquid. It was systematically investigated how anisotropy, i.e. elongation, and quadrupole momentum influence the transport properties. The reduced elongation L* was varied from 0 to 0.8 and the reduced squared quadrupole momentum Q*2 from 0 to 4, i.e. in the entire range in which parameters for real fluids are expected. The statistical uncertainty of the reported data varies with transport property, for self-diffusion coefficient data the error bars are typically lower than 3 %, for shear viscosity and thermal conductivity they are about 8 and 12 %, respectively.

==> bib7_JCP.tex <==
\begin{thebibliography}{99}

\bibitem{alder1} B.J. Alder, D.M. Gass, and T.E. Wainwright,
Phys. Rev. Lett. \textbf{18}, 988(1967).

\bibitem{alder2} B.J. Alder, D.M. Gass, and T.E. Wainwright, J.
Chem. Phys. \textbf{53}, 3813(1970).

\bibitem{hansen} J.P. Hansen and I.A. McDonald, {\it Theory of Simple Liquids}
(Academic Press, London, 1986).

\bibitem{alder3} B.J. Alder, in C. Ciccotti, and W.G. Hoover (Ed.), {\it Molecular-dynamic simulation
of statistical-mechanical systems} (North-Holland, Amsterdam, 1986).

\bibitem{furtado} P.M. Furtado, G.F. Mazenko, and S. Yip, Phys.
Rev. A \textbf{14}, 869(1976).

\bibitem{keyes} T. Keyes and A.J. Masters, Adv. Chem. Phys. \textbf{58}, 1(1985).

\bibitem{macdowell} L.G. MacDowell, B. Garzon, S. Calero, and S. Lago,
J. Chem. Phys. \textbf{106}, 4753 (1997).

\bibitem{McCabe} C. McCabe, C.W. Manke, and P.T. Cummings, J. Chem. Phys. \textbf{116}, 3339(2002).

\bibitem{erpenbeck1} J.J. Erpenbeck and W.W. Wood, J. Stat. Phys. \textbf{24}, 455(1981).

\bibitem{michels1} J.P.J. Michels and N.J. Trappeniers, Chem. Phys. Lett. \textbf{66}, 20(1979).

\bibitem{michels2} J.P.J. Michels and N.J. Trappeniers, Physica A \textbf{101}, 156(1980).

\bibitem{michels3} J.P.J. Michels and N.J. Trappeniers, Physica A \textbf{104}, 243(1980).

\bibitem{michels4} J.P.J. Michels and N.J. Trappeniers, Physica A \textbf{107}, 158(1981).

\bibitem{michels5} J.P.J. Michels and N.J. Trappeniers, Physica A \textbf{107}, 299(1981).

\bibitem{michels6} J.P.J. Michels and N.J. Trappeniers, Physica A \textbf{116}, 516(1982).

\bibitem{heyes1} D.M. Heyes, J. Phys. Condes. Matter. \textbf{6}, 6409(1994).

\bibitem{heyes2} D.M. Heyes, J. Chem. Phys. Faraday Trans. \textbf{79}, 1741(1983).

\bibitem{stoll1} J. Stoll, J. Vrabec, H. Hasse, and J. Fischer,
Fluid Phase Equilibr. \textbf{179}, 339 (2002).

\bibitem{stoll2} J. Stoll, PhD Thesis, {\it Molecular models for the prediction of thermophysical properties
of pure fluid and mixtures}, Reihe 3, Band 836 (VDI, D\"{u}sseldorf, 2005).

\bibitem{vrabec} J. Vrabec, J. Stoll, and H. Hasse, J. Phys. Chem. B \textbf{105}, 12126(2001).

\bibitem{stolljcp} J. Stoll, J. Vrabec, and H. Hasse, J. Phys. Chem. \textbf{119}, 11396(2003).

\bibitem{vrabec2} J. Vrabec, J. Stoll, and H. Hasse, Mol. Sim. \textbf{31}, 215(2001).

\bibitem{stolla} J. Stoll, J. Vrabec, and H. Hasse, AIChE J. \textbf{49}, 2187-2198(2003).

\bibitem{vrabec3} J. Vrabec, G.K. Kedia, and H. Hasse, Cryogenics \textbf{45}, 253(2005).

\bibitem{fernandez2} G.A. Fern\'{a}ndez, J. Vrabec, and H. Hasse, Int. J. Thermophys. \textbf{26}, 1389(2005).

\bibitem{fernandez3} G.A. Fern\'{a}ndez, J. Vrabec, and H. Hasse, Mol. Sim. \textbf{31}, 787(2005).

\bibitem{graygubb} C.G. Gray and K.E. Gubbins, {\it Theory of molecular fluids, Vol. 1:
Fundamentals} (Clarendon Press, Oxford, 1984).

\bibitem{green} M.S. Green, J. Chem. Phys. \textbf{22}, 398(1954).

\bibitem{kubo} R. Kubo, J. Phys. Soc. Jpn. \textbf{12}, 570(1957).

\bibitem{gubbins1} K.E. Gubbins, in K. Singer (Ed.), {\it Statistical mechanics vol. 1} (The chemical
society, Burlington house, London, 1972).

\bibitem{steele} W.A. Steele, in H.J.M. Hanley, (Ed.), {\it Transport phenomena in
fluids} (Marcel Dekker, New York and London, 1969).

\bibitem{baron} A.F.M. Baron, {\it The dynamic liquid state} (Longman, London, 1974).

\bibitem{evans1} D.J. Evans and W.B. Streett, Mol. Phys. \textbf{36}, 161(1978).

\bibitem{vega} C. Vega, S. Lago, E. de Miguel, and L.F. Rull, J. Phys. Chem. \textbf{96}, 7431(1992).

\bibitem{lustig} R. Lustig, Mol. Phys. \textbf{65}, 175(1988).

\bibitem{strett} W.B. Streett and D.J. Tildesley, Proc. R. Soc. A \textbf{355}, 239(1977).

\bibitem{haile} J.M. Haile, {\it Molecular Dynamics Simulation} (John Wiley \& Sons,
New York, 1997).

\bibitem{levesque1} D. Levesque, L. Verlet, and J. K\"{u}rkijarvi, Phys. Rev. A \textbf{7}, 1690(1973).

\bibitem{schoen} M. Schoen and C. Hoheisel, Mol. Phys. \textbf{56}, 653(1985).

\bibitem{erpenbeck2} J.J. Erpenbeck, Phys. Rev. A \textbf{2}, 2514(1974).

\bibitem{fernandezt} G.A. Fern\'{a}ndez, {\it Transport
properties of polar fluids by molecular simulation}, PhD Thesis, University of Stuttgart
(2006).

\bibitem{levesque2} D. Levesque and L. Verlet, Phys. Rev. A \textbf{2}, 2514(1970).

\bibitem{singer} K. Singer, J.V.L. Singer, and A.J. Taylor, Mol. Phys.
\textbf{37}, 1239(1979).

\bibitem{tokumasu} T. Tokumasu, T. Ohara, and K. Kamijo, J. Chem. Phys. \textbf{118}, 3677(2003).

\bibitem{slyusar1} V.P. Slyusar, V.M. Tretyakov, and N.S. Rudenko, Sov. J. Low. Tem. Phys. \textbf{1}, 556(1975).

\bibitem{slyusar2} V.P. Slyusar, V.M. Tretyakov, and N.S. Rudenko, Sov. J. Low. Tem. Phys. \textbf{4}, 363(1978).


\end{thebibliography}

